Named Data Networking for Content Delivery Network Workflows

In this work we investigate Named Data Networking's (NDN's) architectural properties and features, such as content caching and intelligent packet forwarding, in the context of a Content Delivery Network (CDN) workflows. More specifically, we evaluate NDN's properties for PoP (Point of Presence) to PoP and PoP to device connectivity. We use the Apache Traffic Server (ATS) platform to create an HTTP, CDN-like caching hierarchy in order to compare NDN with HTTP-based content delivery. Overall, our work demonstrates that properties inherent to NDN can benefit content providers and users alike. Our experimental results demonstrate that HTTP is faster under stable conditions due to a mature software stack. However, NDN performs better in the presence of packet loss, even for a loss rate as low as 0.1%, due to packet-level caching in the network and fast retransmissions from close upstreams and fast retransmissions from close upstreams. We further show that the Time To First Byte (TTFB) in NDN is consistently lower than HTTP (~100ms in HTTP vs ~50ms in NDN), a vital requirement for CDNs, in addition to supporting transparent failover to another upstream when a failure occurs in the network. Moreover, we examine implementation agnostic (implementation choices can be Software Defined Networking, Information Centric Networking, or something else) network properties that can benefit CDN workflows.

==> 3.1-motivation.tex <==
\section{Motivation}

The current TCP/IP paradigm is end-to-end. On the contrary, the CDNs aim to deliver content in a way that is transparent to the user. Creating a location transparent overlay on top of an end-to-end protocol stack requires hiding several end-to-end artifacts from the users. For example, when using TCP, end to end connections need to be established, even when the transfer size is small. Upstream hosts (caches and origins) need to be enumerated and monitored continuously, and the requests need to be routed to them. When an upstream host fails, a TCP session needs to restart, potentially throwing away already retrieved content. On the contrary, NDN automatically provides a hop-by-hop packet forwarding as well as location independent data retrieval. Since NDN's network model perfectly aligns with CDN's application model, our motivation is to explore these synergies. 

==> notes.tex <==
%\author{Rahul Chatterjee}
%\affiliation{\small{UW--Madison}}


\todo{Take a look at these two papers}:


1. nCDN: CDN enhanced with NDN

2. A tentative comparison on CDN and NDN

3. Experimental Evaluation of Content Distribution with NDN and HTTP


\date{}

In this work we explore Named Data Networking's (NDN) applicability to large scale CDNs. 

\todo[inline]{
%we will write this last
\textbf{Whats the goal?}\\
Large commercial CDNs are optimized for content delivery to millions of users at scale. One key aspect CDNs rely on is performant PoP to PoP connectivity which is used for cache fill in case of cache misses (origin shielding). 
We want to evaluate if NDN can play role in PoP to PoP connectivity by taking advantage of its ability to fetch content from multiple upstreams and graceful failover across different interfaces. \\

\textbf{Things we need to compare against:}\\
1. HTTP bytes range requests from multiple caches\\
2.  Point out differences from multi-path TCP and other Layer 2/3 MPLS load balancing -  In both these cases, you leverage different network paths to the \emph{same} upstream cache/PoP. What we want is application layer seemless failover to other caches. - (Discussion) \\
3.  Not the most crictical, but would be nice to compare against QUIC. - Check\\

\textbf{Key results to show:}\\
0. Without loss/failure NDN has lower TTFB. Lower throughput, higher flow completion times.
1. HTTP failover scenarios and distribution of time to first byte (TTFB), Flow completion times, and for a video stream perfromance metrics like start up delays and rebufferings.\\
1.1 - Fetch files, kill intermediate randomly, run for 10 (1000) times, and get the average cache utilization across all caches.
1.2 - Fetch a video chunk and compare statistics when there is loss

2. Perform same measurements using NDN overlay and show where HTTP wins and where NDN wins. It would be nice to loop over many different file sizes to cover most ground. At the same time keep changing loss and delay parameters.\\
3. One key outcome of this work can be to produce `when' to change upstream cache? For a proactive model, you'd want to have a logic that looks at throughput, loss, etc and decides when to start talking to another cache. Show how exactly NDN can aid the proactive component.\\
4. CDNs often have to worry about millions of flows, showing one fast NDN flow perform better than HTTP is not enough. Show some results of congestion algorithms and their fairness, ability to scale up etc.\\
}

\url{https://docs.trafficserver.apache.org/en/latest/admin-guide/plugins/cache_range_requests.en.html}

